Gaining Explainability from a CNN for Stereotype Detection Based on Mice Stopping Behavior

Understanding the behavior of laboratory animals is a key to find answers about diseases and neurodevelopmental disorders that also affects humans. One behavior of interest is the stopping, as it correlates with exploration, feeding and sleeping habits of individuals. To improve comprehension of animal's behavior, we focus on identifying trait revealing age/sex of mice through the series of stopping spots of each individual. We track 4 mice using LiveMouseTracker (LMT) system during 3 days. Then, we build a stack of 2D histograms of the stop positions. This stack of histograms passes through a shallow CNN architecture to classify mice in terms of age and sex. We observe that female mice show more recognizable behavioral patterns, reaching a classification accuracy of more than 90%, while males, which do not present as many distinguishable patterns, reach an accuracy of 62.5%. To gain explainability from the model, we look at the activation function of the convolutional layers and found that some regions of the cage are preferentially explored by females. Males, especially juveniles, present behavior patterns that oscillate between juvenile female and adult male.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}
 
Understanding behavior in laboratory animals is key to find answers about neurodevelopmental troubles such as autism, schizophrenia and depression. One behavior of interest is the stopping, because it correlates with exploration, nutrition and sleeping habits of individuals. That is why we focus this work on identifying stereotypical traits of individuals through the series of stopping spots of each animal. We track 4 mice using LiveMouseTracker (LMT) system for 3 days. Then, we build a stack of 2D histograms of the stop positions. This stack of histograms pass through a shallow CNN architecture to classify mice in terms of age and sex. We observe that female mice show more distinguishable steretyped pattern, allowing an accuracy in classification of more than 80\%, while males do not present such neat patterns and accuracy drops to 33.3\%. To gain explainability from the model, we look at the activation function of the convolutional layers and found that some regions of the cage are preferentially explored from females. Males, in special juveniles, present behavior patterns that swing between juvenile female and male adult.

\keywords{Automated Behavior Analysis \and Machine Learning \and Animal Tracking}

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%1 what is the main point of our paper
%2 what are the reasons to study this
%3 What methodology approach are we using and why
%4 What are our contributions

Automated Animal Behavior Analysis is a field of study gaining force in the last decade. It has been furnished with increasingly powerful algorithms by computer vision and machine learning in the last few decades. With the possibility of recording experiments with laboratory animals, the manual analysis became obsolete and unfeasible for a human, once the amount of data is beyond the capacity of processing. In special, manual annotations are prone to experimenter bias and drift throughout the annotation process. Thus, researchers have proposed algorithmic solutions to tackle tasks as tracking, identity retention and behavior detection. The animals concerned vary from fruit flies  \cite{eyjolfsdottir2014detecting} to zebrafish \cite{xu2017lie}, ants \cite{khan2005mcmc}, mice \cite{lai20113d,burgos2012social} and many others. 

Understanding behavior in laboratory animals is key to the discovery of disease mechanisms, neural correlations to behaviors and efficient treatments, which can be later tested in humans. That is why it is so important to have consistent analysis protocols and metrics. Although many proposed algorithmic solutions tackle different problems in the field, such as tracking, identity retention and behavior detection, the recognition of impaired and stereotyped behaviors is still a work in progress, with laboratories often arriving to conflicting conclusions.

In general, experiments are designed to have a minimal population of animals that allows statistical significance to tests, but this population is very often not enough to train a deep learning model to detect differences between individuals. Thus, automatic methods capable of reliably highlighting behavioral differences in animals would represent a new step towards understanding stereotypes in neuroscience.

Here, we propose a pipeline to recognize mice age and sex, using the series of stopping points of each individual. The stops spots of the mice in the cage are related to exploration, food and water consumption and sleeping patterns. Our hypothesis is that stereotypical traits can be found on the temporal sequence of stops, because of the different dominance strategies employed by individuals in each gender and age, which affects exploration, nutrition, and sleeping behaviors of individuals. Using the Live Mouse Tracker (LMT) tracking system \cite{de2019real}, we recorded the position and identity and a set of behaviors of multiple cages of four house-grouped mice for 3 days. Then, with a concatenation of single layers Convolutional Networks, we can show that stopping spots sequences actually hides relevant information about animal characteristics and can be enough to predict age and sex of individuals.


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:sota}
%1 Which works do we have in the domain
%2 What did they do to solve the problems (advantages)
%3 what still needs to improve (drawbacks)
%4 what do we do to tackle this problems

Many approaches were already proposed to distinguish animals of different sex, ages or disease conditions, mostly based on social interactions. Mice are particularly studied because of the facility of building disease and neurodevelopmental troubles models similar to human. 
Burgos-Artizzu \textit{et al.} \cite{burgos2012social} proposed a classifier of behavior for a dataset of mice in resident-intruder interactions. The approach is based on spatio-temporal energy and agent trajectories that are used to classify behavior in 13 classes using AdaBoost classifiers. 
York \textit{et al.} \cite{york_flexible_2020} on their turn, presented a pipeline based on postural and displacement features to predict a sequence of behaviors and find neural correlation with movement patterns. 

Netset \textit{et al.} \cite{netser_novel_2017}, for example, presented a new tracking system for analysis of social preference dynamics, and highlight that a loss of social preference is observable in females. The time passed in investigation of the novel individual reduces over time for female, while male keep investigating the new mice up to 5 minutes after introduction.
Zilkha \textit{et al.} \cite{zilkha_sex-dependent_2023} studied the behavioral personalities in male and female mice cages to conclude that, although male and female both establish dominance, each sex has its own strategies. The authors used more than 40 behaviors to build a manifold space, which was reduced to a 3-dimensional space using PCA. Then, differences between male and female, wild and laboratory mice were observed in the distribution of individuals in this feature space.
Finally, Clein \textit{et al.} \cite{clein_automated_2024} investigated dominance hierarchies in mixed-sex groups of mice. Through the detection of sequences of behaviors, the authors showed that the submissive mouse has a mechanism to de-escalate social conflicts.

Despite these findings, none of these works tried to infer individuals' sex, strain or hierarchy, based on the extracted features. Neither of them intended to unveil distinctive features at the individual level that could identify patterns in the animals related to any of the stereotypes studied. In this work, we tackle this particular problem: identify stereotypes on individuals through the series of stopping spots of each animal.

==> sec/3_method.tex <==
\section{Methods}
\label{sec:methods}
%1 Explain the modelling
%2 Describe setup/protocol/dataset
%3 Explain the method
%4 highlight innovations

In the context of a larger work, we recorded 24 male and 24 female mice for 3 days, at two different ages: the first recording around 40 days of life, and the second around 4 months. Animals were housed in groups of four. The recordings were done into a 50x50 cage with food and water \textit{ad libitum}. A system called Live Mouse Tracker (LMT) \cite{de2019real} was used to manage recordings and to retrieve position (center of mass) of mice into the cage at 30 fps. Based on these positions and defining the animals as stopped if its velocity is $\leq$ 5 cm/s, we retrieve all stopping spots in which the mouse remained for at least 1 s. This allowed us to have stop detections consistent with what is seen in video recordings.

The set of stops can be modeled as an irregular time series, since events do not happen in regular intervals, neither in equal quantities for each animal. Figure \ref{fig:irregular_ts} illustrates it. In order to have regular and equally sized information about all the individuals, we compute a histogram of stopping spots. Firstly, the cage surface is split in a regular grid of size $(N\times N)$. Also, data is split in $T$ regular intervals. Then, we count the number of stop events $\mathbb{S}^{t} \in \mathds{R}^{N\times N}$ happening at a tile $\{b_x, b_y\}=\{\left[1\ ...\ N\right], \left[1\ ...\ N\right]\}$ of the grid for each interval $t = \left[ 1\ ...\ T\right]$. Thus, we have a stack of histograms $\mathbf{S} = [\mathbb{S}^{1}; ...\  \mathbb{S}^{T}] \in \mathds{R}^{T \times N \times N}$ representing each individual. These histograms are the features themselves that allow us to distinguish animals and to recognize stereotypes. They represent the evolution in time of the spots' preferences of each individual throughout the experiment. We process these sets of histograms as stacked 2D maps, characterizing the behavior of the animal. An example of such maps is shown in Figure \ref{fig:histogram}. 

\begin{figure}
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{img/timeseries.png}
        \caption{Blue is the position in the x-axis, and green is the position on the y-axis. Markers indicate the initial time of the stop bout.}
        \label{fig:irregular_ts}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.49\textwidth}
        \includegraphics[width=\textwidth]{img/history3.png}
        \caption{Stop spots over time. The clearer the marker, the further in time. The yellow grid shown is the grid created over the cage coordinates.}
        \label{fig:cage}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \includegraphics[scale=0.5]{img/histogram.png}
        \caption{A histogram map of the stop spots. The lighter, the higher is the number of stops in this spot. Here, the mouse spent most of its time in a dome installed in the cage.}
        \label{fig:histogram}
    \end{subfigure}
    \caption{An example of a 1-hour time series of stops of one animal. The most often visited spots are the nest and the feeders.}
    \label{fig:data}
\end{figure}



We build a simple CNN architecture. It is composed of 2 convolutional layers receiving as input the histogram maps. The channels of both layers are flattened and concatenated to pass through a single linear layer. Figure \ref{fig:cnn} illustrates the chosen architecture. The choice of such a network has two goals: Avoid overfitting due to the reduced size of the dataset, and extract explainability of the model choices through the convolution kernel outputs assessment. We train the model to classify data into 4 classes: \texttt{adult-males}, \texttt{juvenile-males}, \texttt{adult-females} and \texttt{juvenile-females}. 
%We also tested the classification into \texttt{male} x \texttt{female} and \texttt{adult} x \texttt{juvenile}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{img/cnn.pdf}
    \caption{CNN architecture developed to predict sex and age from histogram maps of mice}
    \label{fig:cnn}
\end{figure}

==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

%1 describe implementation details
%2 present and discuss results

For the construction of the histogram maps, stoppin spots series were split in $T=72$ 1-hour intervals. The grid over the cage was of $N=30$ tiles. The implemented network was composed of two convolutional layers and ReLU as an activation function. Each layer had different kernel sizes of ($3\times 3$) and ($9\times 9$), both with 16 channels. Output of both layers are subsampled with a Max-pooling layer and then, flattened and concatenated to be sent to a single linear layer for classification. Learning was done with a Cross Entropy Loss, using an SGD optimizer, and learning rate was set to $1e^{-4}$. 

As we observed that maps from mice of the same cage had strong common traits, we adopted a more challenging learning strategy: Dataset is separated per cages and trained using a leave-one(cage)-out cross validation strategy. This avoids the model to rely on common cage features to recognize gender or age, forcing it to learn from generalizing the dynamic features of other cages.

We see the classification results in Table \ref{tab:4class}. We immediately see that juvenile males are completed misclassified as male adults or female-juvenile. 
%Looking at tables \ref{tab:sex} \ref{tab:age}, where training was re-executed to the simplified classes on sex and age, we can see that sex is overall well classified while age show a bias towards the \texttt{adult} class. 
%Samples that are misclassified are majoritarian \texttt{males-juveniles}. 
Looking at the table, we observe that \texttt{juvenile-males} are misclassified as \texttt{juvenile-females}, meaning that they share some patterns up to maturation. We also realize that the model struggles to separate adult and juvenile male mice. This seems an indicative that male mice take more time to transit from juvenile age to adulthood, which justifies the same displacement patterns at both ages, although few \texttt{adult-males} are misclassified as \texttt{juvenile-female}. On the other hand, females had a distinguishable shift in behavior between the two ages.

\begin{table}
    \centering
    \begin{tabular}{ccr|r|r|r}
    \multicolumn{2}{c}{}        & \multicolumn{4}{c}{Pred} \\ 
                           &    & MA & MJ & FA& FJ \\ \cline{3-6}
    \multirow{5}{*}{Labels}& MA & 12 &10 &  0 & 2  \\ \cline{3-6}
                           & MJ & 11 & 4 &  1 & 8  \\ \cline{3-6}
                           & FA &  0 & 4 & 17 & 3  \\ \cline{3-6}
                           & FJ &  0 & 2 &  0 & 22 \\ 
    \end{tabular}
    \caption{Confusion matrix of sex-age classification. Average accuracy is 57.3\%, but accuracy is better among females (81.2\%) than males (33.3\%).}
    \label{tab:4class}
\end{table}
%\begin{table}
%    \centering
%    \begin{tabular}{ccr|r}
%        \multicolumn{2}{c}{}      & \multicolumn{2}{c}{Pred} \\ 
%                                 & &  M &  F \\ \cline{3-4}
%        \multirow{3}{*}{Labels}& M & 40 &  8 \\ \cline{3-4}
%                               & F &  6 & 42 \\
%    \end{tabular}
%    \caption{Confusion matrix of sex classification}
%    \label{tab:sex}
%\end{table}

%\begin{table}
%    \centering
%    \begin{tabular}{ccr|r}
%        \multicolumn{2}{c}{}      & \multicolumn{2}{c}{Pred} \\ 
%                                 & &  A &  J  \\ \cline{3-4}
%        \multirow{3}{*}{Labels}& A & 25 &  23 \\ \cline{3-4}
%                               & J & 11  & 37 \\
%    \end{tabular}
%    \caption{Confusion matrix of age classification}
%    \label{tab:age}
%\end{table}
\vspace{-20pt}

Given these results, we look to the activation maps of the convolution kernels in the network. In Figure \ref{fig:maps}, we see the average over each class of the activation maps for a few channels of the convolutional layer. We can see that kernels learned quickly how to distinguish adult male and female mice, and there's actually no misclassification between them. Activation maps are exactly opposite one to another. While adult females have a strong predilection for the region where a dome was installed, the adult males seem to correlate much less with the same region.

We also see that males correlates more with the lower part of the cage, especially between the lower feeder and the water spot, although adult females also show a similar pattern slightly displaced to the left. 
It's worth noting that no relevant features are observed in juvenile males with relation to other groups, in general it has either the features of adult males or juvenile females (see figures \ref{fig:maps1} and \ref{fig:maps2}), which justify the strong level of misclassification in this class. This suggests that juvenile mice may take more time to mature and that their stopping behavior choices in juvenile age are still not modulated by sexual differences.

\begin{figure}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{img/output_k2_sep_m-f_3.png}
        \caption{}
        \label{fig:maps3}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{img/output_k2_sep_m-f_2.png}
        \caption{}
        \label{fig:maps4}
    \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{img/output_k1_sep_f_adt-juv.png}
        \caption{}
        \label{fig:maps1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{img/output_k1_sep_m_adt-f_juv.png}
        \caption{}
        \label{fig:maps2}
    \end{subfigure}    
    \caption{Activation maps of a few channels of the convolution layers averaged over animals of the same class. red crosses highlights the spots where we see considerable difference between activation maps. Classes are indicated on top of each image. In (a) and (b) it is possible to observe quite distinctive patterns between male and female mice. Patterns are strongly related to upper left corner of the cage, where the dome is placed. In (c) an activation pattern change between adult and juvenile female can be seen. Male maps are similar and response is particularly high in the lower border of the cage, which is also visible in (a) and (d). In (d), adult male and juvenile female maps are particularly different with opposed activations, while juvenile male map seeps to be a fusion of both. }
    \label{fig:maps}
\end{figure}


==> sec/5_conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}

%1 What did we studied
%2 Where did we reach
%3 drawbacks
%4 next steps

In this work, we proposed a concatenation of single layer convolutional network to identify sex and age of animals based on stopping spots over time. Our work shows that, while female have more straightforward identifiable features, stopping spots did not show distinctive features on males over age.

Observation of activation maps helped in understanding which features are more decisive in classification and may help in focusing behavioral analysis on what do mice actually do in these regions. The firsts cues indicates that sleeping and nutrition patterns are the ones that distinguish sex, while the age features are still a challenge for further work.

As next steps, we propose to keep investigating the stopping spots time series in the cage level, to determine which traits correlate with the hierarchy and main stereotypes of dominant/submissive individuals, as well as the variability of these traits with age and sex.
